Higher Tur\'{a}n inequalities for the plane partition function

Here we study the roots of the doubly infinite family of Jensen polynomials $J_{\mathrm{PL}}^{d,n}(x)$ associated to MacMahon's plane partition function $\mathrm{PL}(n)$. Recently, Ono, Pujahari, and Rolen proved that $\mathrm{PL}(n)$ is log-concave for all $n\geq 12$, which is equivalent to the polynomials $J_{\mathrm{PL}}^{2,n}(x)$ having real roots. Moreover, they proved, for each $d\geq 2$, that the $J_{\mathrm{PL}}^{d,n}(x)$ have all real roots for sufficiently large $n$. Here we make their result effective. Namely, if $N_{\mathrm{PL}}(d)$ is the minimal integer such that $J_{\mathrm{PL}}^{d,n}(x)$ has all real roots for all $n\geq N_{\mathrm{PL}}(d)$, then we show that $$N_{\mathrm{PL}}(d)\leq 279928\cdot d(d-1)\cdot \left(6 d^3\cdot (22.2)^{\frac{3(d-1)}{2}}\right)^{2d} e^{\frac{\Gamma(2d^2)}{(2\pi)^{2d+2}}} .$$ Moreover, using the ideas that led to the above inequality, we explicitly prove that $N_{\mathrm{PL}}(3)=26, N_{\mathrm{PL}}(4)=46, N_{\mathrm{PL}}(5)=73, N_{\mathrm{PL}}(6)=102$ and $N_{\mathrm{PL}}(7)=136$.

==> Tex file 2/main.tex <==
@misc{ono2022turan,
      title={Tur\'an inequalities for the plane partition function}, 
      author={Ken Ono and Sudhir Pujahari and Larry Rolen},
      year={2022},
      eprint={2201.01352},
      archivePrefix={arXiv},
      primaryClass={math.NT}
}

@article{larson2019,
	title={Hyperbolicity of the partition Jensen polynomials},
	author={Larson, Hannah and Wagner, Ian},
	year={2019},
	journal={Research in Number Theory},
	volume = {5},
	doi= {10.1007/s40993-019-0157-y},
	ID = {Larson2019},
	SN = {2363-9555},
	UR = {https://doi.org/10.1007/s40993-019-0157-y}
}

@article{jensen1913,
TYPE  = {JOURNAL},
AUTHOR  = {Jensen, J. L. W. V.},
YEAR  = {1913},
DATE  = {1913/12/01},
title  = {Recherches sur la théorie des équations},
journal  = {Acta Mathematica},
SP  = {181},
EP  = {195},
VOLUME  = {36},
IS  = {1},
SN  = {1871-2509},
UR  = {https://doi.org/10.1007/BF02422380},
DO  = {10.1007/BF02422380},
ID  = {Jensen1913} 
}

@article{griffin2019,
doi={10.1073/pnas.1902572116},
author = {Michael Griffin  and Ken Ono  and Larry Rolen  and Don Zagier },
title = {Jensen polynomials for the Riemann zeta function and other sequences},
journal = {Proceedings of the National Academy of Sciences},
volume = {116},
number = {23},
pages = {11103-11110},
year = {2019},
doi = {10.1073/pnas.1902572116},
URL = {https://www.pnas.org/doi/abs/10.1073/pnas.1902572116},
eprint = {https://www.pnas.org/doi/pdf/10.1073/pnas.1902572116},
abstract = {The Pólya–Jensen criterion for the Riemann hypothesis asserts that RH is equivalent to the hyperbolicity of certain Jensen polynomials for all degrees d≥1 and all shifts n. For each degree d≥1, we confirm this criterion for all sufficiently large shifts n. This represents a theoretical advance in the field. The method of proof is rooted in the newly discovered phenomenon that these polynomials are nicely approximated by Hermite polynomials. Furthermore, it is shown that this method applies to a large class of related problems. In 1927, Pólya proved that the Riemann hypothesis is equivalent to the hyperbolicity of Jensen polynomials for the Riemann zeta function ζ(s) at its point of symmetry. This hyperbolicity has been proved for degrees d≤3. We obtain an asymptotic formula for the central derivatives ζ(2n)(1/2) that is accurate to all orders, which allows us to prove the hyperbolicity of all but finitely many of the Jensen polynomials of each degree. Moreover, we establish hyperbolicity for all d≤8. These results follow from a general theorem which models such polynomials by Hermite polynomials. In the case of the Riemann zeta function, this proves the Gaussian unitary ensemble random matrix model prediction in derivative aspect. The general theorem also allows us to prove a conjecture of Chen, Jia, and Wang on the partition function.}}

@article{GRIFFIN2022108186,
title = {Jensen polynomials for the Riemann xi-function},
journal = {Advances in Mathematics},
volume = {397},
pages = {108186},
year = {2022},
issn = {0001-8708},
doi = {https://doi.org/10.1016/j.aim.2022.108186},
url = {https://www.sciencedirect.com/science/article/pii/S0001870822000020},
author = {Michael J. Griffin and Ken Ono and Larry Rolen and Jesse Thorner and Zachary Tripp and Ian Wagner},
keywords = {Riemann zeta function, Riemann hypothesis, Jensen polynomial},
abstract = {We investigate ξ(s)=12s(s−1)π−s2Γ(s2)ζ(s), where ζ(s) is the Riemann zeta function. The Riemann hypothesis (RH) asserts that if ξ(s)=0, then Re(s)=12. Pólya proved that RH is equivalent to the hyperbolicity of the Jensen polynomials Jd,n(X) constructed from certain Taylor coefficients of ξ(s). For each d≥1, recent work proves that Jd,n(X) is hyperbolic for sufficiently large n. In this paper, we make this result effective. Moreover, we show how the low-lying zeros of the derivatives ξ(n)(s) influence the hyperbolicity of Jd,n(X).}
}

@book{polya1927,
author={P\'olya, George},
title = {Uber die algebraisch-Funktionentheoretische Untersuchungen von J.L.W.V. Jensen},
publisher = {A.F. Hst},
volume = {},
pages = {},
year = {1927},
}

==> main.tex <==
@misc{ono2022turan,
      title={Tur\'an inequalities for the plane partition function}, 
      author={Ken Ono and Sudhir Pujahari and Larry Rolen},
      year={2022},
      eprint={2201.01352},
      archivePrefix={arXiv},
      primaryClass={math.NT}
}

@article{larson2019,
	title={Hyperbolicity of the partition Jensen polynomials},
	author={Larson, Hannah and Wagner, Ian},
	year={2019},
	journal={Research in Number Theory},
	volume = {5},
	doi= {10.1007/s40993-019-0157-y},
	ID = {Larson2019},
	SN = {2363-9555},
	UR = {https://doi.org/10.1007/s40993-019-0157-y}
}

@article{jensen1913,
TYPE  = {JOURNAL},
AUTHOR  = {Jensen, J. L. W. V.},
YEAR  = {1913},
DATE  = {1913/12/01},
title  = {Recherches sur la théorie des équations},
journal  = {Acta Mathematica},
SP  = {181},
EP  = {195},
VOLUME  = {36},
IS  = {1},
SN  = {1871-2509},
UR  = {https://doi.org/10.1007/BF02422380},
DO  = {10.1007/BF02422380},
ID  = {Jensen1913} 
}

@article{griffin2019,
doi={10.1073/pnas.1902572116},
author = {Michael Griffin  and Ken Ono  and Larry Rolen  and Don Zagier },
title = {Jensen polynomials for the Riemann zeta function and other sequences},
journal = {Proceedings of the National Academy of Sciences},
volume = {116},
number = {23},
pages = {11103-11110},
year = {2019},
doi = {10.1073/pnas.1902572116},
URL = {https://www.pnas.org/doi/abs/10.1073/pnas.1902572116},
eprint = {https://www.pnas.org/doi/pdf/10.1073/pnas.1902572116},
abstract = {The Pólya–Jensen criterion for the Riemann hypothesis asserts that RH is equivalent to the hyperbolicity of certain Jensen polynomials for all degrees d≥1 and all shifts n. For each degree d≥1, we confirm this criterion for all sufficiently large shifts n. This represents a theoretical advance in the field. The method of proof is rooted in the newly discovered phenomenon that these polynomials are nicely approximated by Hermite polynomials. Furthermore, it is shown that this method applies to a large class of related problems. In 1927, Pólya proved that the Riemann hypothesis is equivalent to the hyperbolicity of Jensen polynomials for the Riemann zeta function ζ(s) at its point of symmetry. This hyperbolicity has been proved for degrees d≤3. We obtain an asymptotic formula for the central derivatives ζ(2n)(1/2) that is accurate to all orders, which allows us to prove the hyperbolicity of all but finitely many of the Jensen polynomials of each degree. Moreover, we establish hyperbolicity for all d≤8. These results follow from a general theorem which models such polynomials by Hermite polynomials. In the case of the Riemann zeta function, this proves the Gaussian unitary ensemble random matrix model prediction in derivative aspect. The general theorem also allows us to prove a conjecture of Chen, Jia, and Wang on the partition function.}}

@article{GRIFFIN2022108186,
title = {Jensen polynomials for the Riemann xi-function},
journal = {Advances in Mathematics},
volume = {397},
pages = {108186},
year = {2022},
issn = {0001-8708},
doi = {https://doi.org/10.1016/j.aim.2022.108186},
url = {https://www.sciencedirect.com/science/article/pii/S0001870822000020},
author = {Michael J. Griffin and Ken Ono and Larry Rolen and Jesse Thorner and Zachary Tripp and Ian Wagner},
keywords = {Riemann zeta function, Riemann hypothesis, Jensen polynomial},
abstract = {We investigate ξ(s)=12s(s−1)π−s2Γ(s2)ζ(s), where ζ(s) is the Riemann zeta function. The Riemann hypothesis (RH) asserts that if ξ(s)=0, then Re(s)=12. Pólya proved that RH is equivalent to the hyperbolicity of the Jensen polynomials Jd,n(X) constructed from certain Taylor coefficients of ξ(s). For each d≥1, recent work proves that Jd,n(X) is hyperbolic for sufficiently large n. In this paper, we make this result effective. Moreover, we show how the low-lying zeros of the derivatives ξ(n)(s) influence the hyperbolicity of Jd,n(X).}
}

@book{polya1927,
author={P\'olya, George},
title = {Uber die algebraisch-Funktionentheoretische Untersuchungen von J.L.W.V. Jensen},
publisher = {A.F. Hst},
volume = {},
pages = {},
year = {1927},
}
